Distributed generation of privacy preserving data with user customization

Distributed devices such as mobile phones can produce and store large amounts of data that can enhance machine learning models; however, this data may contain private information specific to the data owner that prevents the release of the data. We wish to reduce the correlation between user-specific private information and data while maintaining the useful information. Rather than learning a large model to achieve privatization from end to end, we introduce a decoupling of the creation of a latent representation and the privatization of data that allows user-specific privatization to occur in a distributed setting with limited computation and minimal disturbance on the utility of the data. We leverage a Variational Autoencoder (VAE) to create a compact latent representation of the data; however, the VAE remains fixed for all devices and all possible private labels. We then train a small generative filter to perturb the latent representation based on individual preferences regarding the private and utility information. The small filter is trained by utilizing a GAN-type robust optimization that can take place on a distributed device. We conduct experiments on three popular datasets: MNIST, UCI-Adult, and CelebA, and give a thorough evaluation including visualizing the geometry of the latent embeddings and estimating the empirical mutual information to show the effectiveness of our approach.

==> diagram_graph_latent.tex <==
\begin{figure}[!hpbt]
    \centering
    % \includegraphics{}
    % \caption{Caption}
    % \label{fig:my_label}
\begin{tikzpicture}

  % Define nodes
  \node[obs]                               (tilde_z) {$\tilde{z}$};
  \node[latent, above=of tilde_z, xshift=-1.2cm] (z) {$ {z}$};
  \node[latent, above=of tilde_z, xshift=0.0cm]  (vareps) {$\boldsymbol{\epsilon}$};
  \node[latent, above=of tilde_z, xshift=1.2cm]  (y) {$ {y}$};
%   \node[latent, right=2cm of ]            (t) {$\tau$};

  % Connect the nodes
  \edge {z,vareps,y} {tilde_z} ; %
  %\edge {y} {vareps};

%   % Plates
%   \plate {yx} {(x)(y)} {$N$} ;
%   \plate {} {(w)(y)(yx.north west)(yx.south west)} {$M$} ;

\end{tikzpicture}
\caption{random variable graphic model. In our setting of noise injection on latent space, we yield new latent representation $\tilde{z}$ according to original latent variable $z$, random noise $\epsilon$, and sensitive label $y$.}
\label{fig:diagram:relationship}
\end{figure}

==> discarded/Connection_to_adversarial.tex <==
\section{Connection with adversarial examples}
A typical adversarial training/example problem \cite{raghunathan2018certified,sinha2018certifying, wong2018provable,madry2017towards} can be formulated as the following optimization :
\begin{align}
    \min_{\theta_h}\mathbb{E}_{z, y}\Big( \max_{\tilde{z} \in \mathcal{B}_{\epsilon, p}(z) } \ell(h_{\theta_h}(\tilde{z}), y)\Big) = \min_{\theta_h} \frac{1}{|\mathcal{D}|} \sum_{(z, y) \in \mathcal{D}} \max_{\tilde{z}\in \mathbf{\mathcal{B}}_{\epsilon, p}(z) }\ell(h_{\theta_h}(\tilde{z}), y), 
\end{align}
where $\mathbf{\mathcal{B}}_{\epsilon, p}(z) = \{\tilde{z}: ||\tilde{z} - z ||_p \leq \epsilon \}$ denotes the set of epsilon-$L_p$ ball around point $z$.  The goal, in this context, is to minimize the loss at worst scenario given the dataset $\mathcal{D}$. In other words, this formulation aims to train a robust classifier $h$ parameterized by $\theta_h$ when encountering with  epsilon-$L_p$ ball perturbation. A number of methods have been proposed to solve the inner maximization. The Fast Gradient Sign Method (FGSM) \cite{papernot2017practical}  is maximizing over $L_{\infty}$ ball that yields $\tilde{z} = z + \epsilon \text{\textsf{sign}}\big(\nabla_z \ell(\theta_h, z, y)\big)$. A variant approach is projected gradient method (PGM) \cite{madry2017towards} that can be viewed as ${z}^{(t+1)} = \Pi_{\mathcal{B}_{\epsilon, p}(z^{(t)})}(z^{(t)} + \eta \tilde{v}^{(t)}  )$ where $\tilde{v}^{(t)} = \arg\max_{\|v\|_p \leq \epsilon } (v^T \nabla_{z}\ell(\theta_h; z^{(t)}, y)) $ and $\eta$ is the step size, when iterating from 1 to $T_a$ steps. Then we set $\tilde{z} = z^{(T_a)}$ at the last step $T_a$. 

We use FGSM and PGM restricted on $L_{\infty}$ ball and $L_2$ ball to compare the performance of latent variable perturbations. In this case we explicitly write out the expression 
\begin{align*}
    \tilde{v}^{t} = \begin{cases}
    \frac{\epsilon \nabla_{z}\ell(\theta_h; z^{(t)}, y)}{||\nabla_{z}\ell(\theta_h; z^{(t)}, y)||_2} & p=2 ; \quad (L_2) \\
    \epsilon \text{\textsf{sign}}(\nabla_{z}\ell(\theta_h; z^{(t)}, y)) & p = \infty \quad (L_{\infty}) 
    \end{cases}.
\end{align*}
To give the intuition of why the expression is valid, we provide an informal proof as follows. Let $q$ norm be the dual norm of the $p$ norm ($\frac{1}{p}+\frac{1}{q}=1$). For $p=2$, i.e. $L_2$-norm, by using H$\ddot{\text{o}}$lder's inequality, we have $v^Tx \leq ||v||_p ||x||_q = ||v||_2 ||x||_2 
\leq \epsilon ||x||_2$. Thus the equality holds only when $v=  \frac{\epsilon x}{\|x\|_2}$. Then substituting $x$ with $\nabla_{z}\ell(\theta_h; z^{(t)}, y)$ yields the result. The associate value of $v$ in the case of $L_{\infty}$ can be obtained as applying the similar derivation. 

\textcolor{red}{TODO... add more details}

==> discarded/robust_optimization_chisq.tex <==
p = project\_{onto}\_{chi}\_{square}\_{ball}$(w, \rho, tol = 1e-10)$

 Solves the projection problem given above by bisecting on the dual problem
\begin{align*}
 \max_{\lambda >= 0}  \min_{p}  .5 * ||(p - w||_2^2 - \lambda * (\rho + .5 - .5 * n * ||p||^2) \\
                        s.t.    \sum(p) = 1, p >= 0
\end{align*}
 where we used $(1/nn) * .5 * \sum_{i=1}^n (n * p[i] - 1)^2 = .5 * (n * norm(p)^2 - 1)$
 and duality. The KKT conditions of the inner minimization problem are given by

 $p(\lambda) = (1 / (1 + \lambda * n)) * \max(w - \eta, 0)$

 where eta is the dual variable for the constraint $\sum(p) = 1$. We
 solve eta such that $\sum(p(\lambda)) = 1$ in solve\_inner\_eta.

 Given such eta, first note that the gradient of the dual objective 
\begin{align*}
 g(\lambda) = \min_{p}  .5 * ||(p - w)||_2^2 
                     - \lambda * (\rho + .5 - .5 * n * ||p||_2^2) \\
            s.t.    \sum(p) = 1, p >= 0
\end{align*}
 with respect to lam is given by
 $g'(\lambda) = -(\rho + .5 - .5 * n * norm(p(\lambda))^2)$.

 Since g is concave, $g'$ is decreasing in $\lambda$. Hence, we bisect to find
 the optimal lam:

 If $g'(lam) > 0$,  i.e.$.5 * n * norm(p(lam))^2 > \rho + .5$,  increase lam \\
 If $g'(lam) < 0$,  i.e. $.5 * n * norm(p(lam))^2 < rho + .5$,  decrease lam.


 %-------------- obtaining an finite upper bound for lam^* ---------------

 Note that the optimal dual solution $lam^*$ satisfies
$.5 * n * (1/ (1 + \lambda * n)^2) * \sum (w[i] - eta)^2 = \rho + .5$
 so that this gives the bound
$(1 + \lambda^* * n)^2 <= \max(w)^2 * n^2 / (2 * \rho + 1)$

 or equivalently,

 $\lambda^* <= (1/n) * (n * \max(w) / \sqrt{(2 * \rho + 1)} - 1) := \lambda_{max} .$

 %------------------------------------------------------------------------
